LoRA-GA: Low-Rank Adaptation with Gradient Approximation

Fine-tuning large-scale pretrained models is prohibitively expensive in terms of computational and memory costs. LoRA, as one of the most popular Parameter-Efficient Fine-Tuning (PEFT) methods, offers a cost-effective alternative by fine-tuning an auxiliary low-rank model that has significantly fewer parameters. Although LoRA reduces the computational and memory requirements significantly at each iteration, extensive empirical evidence indicates that it converges at a considerably slower rate compared to full fine-tuning, ultimately leading to increased overall compute and often worse test performance. In our paper, we perform an in-depth investigation of the initialization method of LoRA and show that careful initialization (without any change of the architecture and the training algorithm) can significantly enhance both efficiency and performance. In particular, we introduce a novel initialization method, LoRA-GA (Low Rank Adaptation with Gradient Approximation), which aligns the gradients of low-rank matrix product with those of full fine-tuning at the first step. Our extensive experiments demonstrate that LoRA-GA achieves a convergence rate comparable to that of full fine-tuning (hence being significantly faster than vanilla LoRA as well as various recent improvements) while simultaneously attaining comparable or even better performance. For example, on the subset of the GLUE dataset with T5-Base, LoRA-GA outperforms LoRA by 5.69% on average. On larger models such as Llama 2-7B, LoRA-GA shows performance improvements of 0.34, 11.52%, and 5.05% on MT-bench, GSM8K, and Human-eval, respectively. Additionally, we observe up to 2-4 times convergence speed improvement compared to vanilla LoRA, validating its effectiveness in accelerating convergence and enhancing model performance. Code is available at https://github.com/Outsider565/LoRA-GA.

==> text_part/analysis.tex <==
\section{Analysis}

\subsection{How Low is the Rank of Gradient?}
According to the Theorem \ref{thm:thm_align}, the gradient aligning problem has reached an optimal solution, whose objective is minimized to \( \sum_{i=2r+1}^{\min{\m, \n}} \sigma^2\), where \(\sigma_i\) is the \(i\)-th sigular value from \(S\). Therefore, the closer the rank of the gradient matrix to \(2r\), the better the gradient aligned by \(A_{\mathrm{init}}\) and \(B_{\mathrm{init}}\), and more effective our initialization is theoretically. So that it's necessary to verify the rank of gradients.

In Figure \ref{fig:fig_lowrank}, we show that the rank of gradient matrices is very low. The left one shows the grid-like scale of gradients for a weight matrix, which means that this matrix has a lot of similar rows and columns intuitively. The middle one gives the decreasing curve of singular values of the gradient. Even in the case of the logarithmic horizontal axis, the curve still falls very steeply, implies that the gradient is a highly low-rank matrix. The right one gives the cumulative curve of squared singular values, which indicates that only few ranks can cover almost all singular values of a gradient matrix. 

\begin{figure}
    \centering
    \includegraphics[height = 4.2cm]{img/gradient_matrix.jpg}
    \includegraphics[height = 4.2cm]{img/singular_value.jpg}
    \includegraphics[height = 4.2cm]{img/coverage.jpg}
    \caption{({\bf Left}) Value distribution in a gradient matrix of T5-base on fine-tuning CoLA. It looks like a grid, implies some possible patterns of gradient. ({\bf Middle}) Decreasing curve of singular values of the gradient matrix, suggests it's a highly low-rank matrix. ({\bf Right}) Cumulative curve of the coverage of squared singular values, shows only few ranks can cover almost all singular values of gradient. }
    \label{fig:fig_lowrank}
\end{figure}

All these 3 pictures shows that gradient matrices are highly low-rank, which can be approximated well by low-rank matrices, which firmly supports our idea of gradient alignment.






==> text_part/analysis_of_lora.tex <==
\section{Initialization Analysis of LoRA}
\subsection{Low-Rank Adaptation (LoRA)}
Based on the hypothesis that the updates of fine-tuning is low-rank, LoRA \cite{hu2021lora} proposed to use the product of 2 low-rank matrices to express the incremental part of original parameter $W_0$. To be specific, it has a mathematical form like:
\[
W' = W + \Delta W = W_0 + \dfrac{\alpha}{r} BA := W_0 + \eta BA
\]
where $W', W_0 \in \mathbb{R}^{m\times n} $, $B\in \mathbb{R}^{m\times r} $ and $A \in \mathbb{R}^{r\times n} $, in which $r \ll \min(m, n)$. $W_0$ remains frozen during the fine-tuning process. 

Under LoRA setting, matrix $A$ is initialized with normal distribution, while the matrix $B$ is initialized with all $0$. Therefore, $BA=0$ and $W'_0 = W_0$, keeps the initial point identical. In different settings, $\Delta W$ can be replaced with other variants of LoRA. Specifically, if the additional term $\Delta W_0 = \eta B_0 A_0$ is initially non-zero, the frozen parameter can be adjusted to maintain the initial point unchanged. This can be expressed as:
\begin{align}
    W'_0 = (W_0 - \eta B_0 A_0)_{frozen} + \eta B_0 A_0 := W_{fz} + \eta B_0 A_0
    \label{eq:eq_lora}
\end{align} 
where $W_{fz} = W_0 - \eta B_0 A_0$ is frozen, $B_0$ and $A_0$ is trainable in this case.


\subsection{Gradient Alignment}
\subsubsection{Problem Motivation}
If using LoRA to fine-tune a model, the parameter can be expressed in the form of equation \ref{eq:eq_lora}, and the model will be like:
\[
y = [W_{fz} + \eta B_0 A_0] x
\]
After fine-tuning, the parameter $B_0A_0$ is tuned to $B_{ft}A_{ft}$. Therefore, the update of LoRA is $\eta (B_{ft}A_{ft} - B_0A_0) = \eta \Delta (BA) $.

Under an ideal situation, it's optimal that the LoRA update of parameter $W$ is aligned to the full fine-tuning update, i.e., $\forall k$, we want to solve the optimization problem that:
\begin{align}
    \min_{A_0, B_0} \fnorm{\eta k \Delta (BA) - \Delta {W}}
    \label{eq:eq_ori_prob}
\end{align}
where $k$ is a scaling factor, which can be a function of $m$, $n$ and $r$.

\subsubsection{Problem Settings}
In order to solve problem \ref{eq:eq_ori_prob}, we need to do some hypothesis and simplifications.
\begin{itemize}
    \item The parameters are all updated by SGD optimizer;
    \item The learning rate $\alpha$ is quite small, so that $\alpha^2 = o(1)$, which can be ignored when calculating;
    \item $\fnorm{\Delta W}$, $\fnorm{\Delta A}$ and $\fnorm{\Delta B}$ are all close to $0$. (Because we only care about the dynamics of the beginning of the training.)
\end{itemize}

Thus, problem \ref{eq:eq_ori_prob} can be approximated as:
\begin{align}
    \fnorm{\eta k \Delta (BA) - \Delta {W}}
    &=
    \fnorm{\eta k (\Delta B \cdot A + B \cdot \Delta A) - \Delta W }\\
    &=
    \fnorm{\eta k \left(
    \alpha \dfrac{\partial L}{\partial B} A
    +
    \alpha B \dfrac{\partial L}{\partial A}
    \right)
    -
    \alpha \dfrac{\partial L}{\partial W}
    }\\
    &=
    \alpha\fnorm{\eta k \left(
    \dfrac{\partial L}{\partial B} A
    +
    B \dfrac{\partial L}{\partial A}
    \right)
    -
    \dfrac{\partial L}{\partial W}
    }
    \label{eq:eq_apr_prob}
\end{align}


\begin{align}
    aaa
    \label{eq:eq_align}
\end{align} 


\subsection{Rank and Scale Stability}

\begin{align}
    aaa
    \label{eq:eq_scale}
\end{align}

